Reduced basis methods for quasilinear elliptic PDEs with applications to permanent magnet synchronous motors

In this paper, we propose a certified reduced basis (RB) method for quasilinear elliptic problems together with its application to nonlinear magnetostatics equations, where the later model permanent magnet synchronous motors (PMSM). The parametrization enters through the geometry of the domain and thus, combined with the nonlinearity, drives our reduction problem. We provide a residual-based a-posteriori error bound which, together with the Greedy approach, allows to construct reduced-basis spaces of small dimensions. We use the empirical interpolation method (EIM) to guarantee the efficient offline-online computational procedure. The reduced-basis solution is then obtained with the surrogate of the Newton's method. The numerical results indicate that the proposed reduced-basis method provides a significant computational gain, compared to a finite element method.

==> latexmkrc <==
$makeindex  = 'makeindex -s svind.ist %O -o %D %S';

# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"

% Journal article
\bibitem{science-journal} Alla, A., Hinze, M., Kolvenbach, P. et al. A certified model reduction approach for robust parameter optimization with PDE constraints. Adv Comput Math \textbf{45}, 1221–1250 (2019). 
% Journal article
\bibitem{science-journal} Ion, I.G., Bontinck, Z., Loukrezis, D. et al. Robust shape optimization of electric devices based on deterministic optimization methods and finite-element analysis with affine parametrization and design elements. Electr Eng \textbf{100}, 2635–2647 (2018).

\bibitem{science-journal} Bachinger, F., Langer, U. & Schöberl, J. Numerical analysis of nonlinear multiharmonic eddy current problems. Numer. Math. 100, 593–616 (2005)

\bibitem{science-journal} Barrault, M., Maday, Y., Nguyen, N.C., Patera, A.T.: An empirical interpolation method: application to efficient reduced-basis discretization of partial differential equations. C.R. Acad.Sci.Paris Ser.I \textbf{339}(9), 667-672 (2004)
% Journal article
\bibitem{science-journal} Grepl, M.A., Maday, Y., Nguyen, N.C., Patera, A.T.: Efficient reduced-basis treatment of nonaffine and nonlinear partial differential equations. ESAIM: Math. Mod. and Num. Anal. \textbf{41}(3), 575-605, 2007
% Journal article
\bibitem{science-journal} Lass, O., Ulbrich, S.: Model order reduction techniques with a posteriori error control for nonlinear robust optimization governed by partial differential equations. SIAM J. on Sc. Comp. \textbf{39}, S112-S139 (2017)
% Journal article
\bibitem{science-journal} Rozza, G., Huynh, D.B.P., Patera, A.T.: Reduced basis approximation and a posteriori error estimation for affinely parametrized elliptic coercive partial differential equations. Arch. Comput. Methods Eng. \textbf{15}, 229-275 (2008)
% Journal article
\bibitem{science-journal} Rozza, G., Huynh, D.B.P., Patera, A.T.: Reduced basis approximation and a posteriori error estimation for affinely parametrized elliptic coercive partial differential equations. Arch. Comput. Methods Eng. \textbf{15}, 229-275 (2008)
% Journal article
\bibitem{science-journal} Heise, B.: Analysis of a fully discrete finite element method for a nonlinear magnetic field problem. SIAM J. Num. Anal. \textbf{31}(3), 745-759 (1994)
% Tutorial 
\bibitem{science-contrib} Haasdonk, B.: Reduced basis methods for parametrized PDEs - a tutorial introduction for stationary and instationary problems. In: Benner, P., Cohen, A., Ohlberger, M., Willcox, K. (eds.) Chapter in Model Reduction and Approximation: Theory and Algorithms, pp. 65-136. SIAM, Philadelphia (2007)
% Monograph
\bibitem{science-mono} Zeidler, E.: Nonlinear Functional Analysis and Its Applications: II/B: Nonlinear Monotone Operators. Springer Science & Business Media, New York (1990) 
% Monograph
\bibitem{science-mono} Quarteroni, A., Manzoni, A., Negri , F.: Reduced basis methods for partial differential equations: an introduction, vol. 92. Springer International Publishing, Switzerland (2016)


\end{thebibliography}

